SqORAM: Read-Optimized Sequential Write-Only Oblivious RAM

Oblivious RAM protocols (ORAMs) allow a client to access data from an untrusted storage device without revealing the access patterns. Typically, the ORAM adversary can observe both read and write accesses. Write-only ORAMs target a more practical, {\em multi-snapshot adversary} only monitoring client writes -- typical for plausible deniability and censorship-resilient systems. This allows write-only ORAMs to achieve significantly-better asymptotic performance. However, these apparent gains do not materialize in real deployments primarily due to the random data placement strategies used to break correlations between logical and physical namespaces, a required property for write access privacy. Random access performs poorly on both rotational disks and SSDs (often increasing wear significantly, and interfering with wear-leveling mechanisms). In this work, we introduce SqORAM, a new locality-preserving write-only ORAM that preserves write access privacy without requiring random data access. Data blocks close to each other in the logical domain land in close proximity on the physical media. Importantly, SqORAM maintains this data locality property over time, significantly increasing read throughput. A full Linux kernel-level implementation of SqORAM is 100x faster than non locality-preserving solutions for standard workloads and is 60-100% faster than the state-of-the-art for typical file system workloads.

==> abstract.tex <==
\abstract{
Oblivious RAM (ORAM) technology has advanced rapidly.  Under certain client-side
storage assumptions, tree-based ORAM designs \cite{pathoram} have achieved
established lower bounds even for {\em online} adversaries that can monitor
everything a client does.
Write-only ORAMs target a more practical, albeit weaker {\em
multi-snapshot adversary} -- typical in plausible deniability and censorship-resilient
systems~\cite{hive,datalair} -- only monitoring client {\em writes}. 
This allows write-only ORAMs to achieve significantly better asymptotic 
performance. These apparent gains do not materialize in real deployments  
however, primarily due to the random data placement strategies used in 
existing write-only ORAMs to break correlations between logical and physical 
namespaces, a required property for write access privacy.  Random access performs poorly on both rotational disks and SSDs, often increasing wear significantly, and interfering with
wear-leveling mechanisms.
In this work, we introduce {\sys}, a new locality-preserving write-only ORAM
that preserves write access privacy without requiring random data access. 
Data blocks close to each other in the logical domain land in close
proximity on the physical media.  Importantly, {\sys} maintains this data 
locality property over time, significantly increasing read throughput.\\
A full Linux kernel-level implementation of {\sys} is 100x faster
than non locality-preserving solutions for standard workloads, performs comparably 
to the one existing locality-preserving system for writes and outperforms 
it for reads by \todo{how much in percent \%} 
% faster than the state-of-the-art for a typical mail server workload.
% and is only 1.5x slower than a baseline block device implementation with no access privacy.
}



==> algo.tex <==
\section{Algorithms}
%


\begin{algorithm}[th!]
	\caption{$\mathsf{merge(i)}$}\label{merge_level}
	\begin{algorithmic}[1]
		\footnotesize
		\item[] $q_w := \phi$ (queue of size $\beta$)
		\item[] $q_m:= \phi$ (queue of size $\beta$)
		\item[] $ctr_{w} := 0$ 
		\item[] $ctr_{m} := 0$ 
		\item[] $ctr_{next} := 0$
		
		\For{x = 1 to $2^{i+1}\beta$}
		%	\If{$q_0.empty$}				
		\While{ $q_w.notFull$}
		\If{$ctr_{w} \leq 2^{i}\beta$}
		\State Enqueue($q_w$, readFromWriteBuffer($i, ctr_{w}$)) 
		\State $ctr_{w} = ctr_{w} + 1$
		\Else
		\State Enqueue($q_w$, fake)
		\EndIf	
		\EndWhile
		%	\EndIf
		%	\If{$q_1.empty$}		
		\While{ $q_m.notFull$}
		\If{$ctr_{m} \leq 2^{i}\beta$}
		\State Enqueue($q_m$, readFromMergeBuffer($i, ctr_{m}$))
		\State $ctr_{m} = ctr_{m} + 1$ 
		\Else
		\State Enqueue($q_m$, fake)
		\EndIf	
		\EndWhile
		%	\EndIf
		
		\For{y = 1 to $\beta$}
		\State $b_0 = q_{0}.peek$
		\State $b_1 = q_{1}.peek$
		%	\If{$i \neq \log{N}$}
		\If {$b_0.add < b_1.add$}
		\State $b$ = Dequeue($q_{0}$)
		\ElsIf {$b_0.add = b_1.add$}
		\State  $b$ = Dequeue($q_{0}$)
		\State (discard $b_1$ from $q_{1}$)
		\Else
		\State $b$ = Dequeue($q_{1}$)
		\EndIf
		\If{$i \neq \log{N}$}
		\State writeNextToWriteBuffer($i+1, ctr_{next}, b$)
		\Else
		\State writeNextToWriteBuffer($i, ctr_{next}, b$)
		\EndIf
		
		%					
		\State $ctr_{next} = ctr_{next} + 1$
		\EndFor
		\EndFor
		%\end{footnotesize}							
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[th!]
	\caption{$\mathsf{merge\_deamortized}$}\label{merge_level_deamortized}
	\begin{algorithmic}[1]
		%\begin{scriptsize}
		\footnotesize
		\Procedure{Init}{$\phi$}
		\item[] $q_{x0} := \phi$ // Persistent in-memory queue of size $\beta$ assigned for level $x < \log{N}$
		\item[] $q_{x1} := \phi$ // Persistent in-memory queue of size $\beta$ assigned for level $x < \log{N}$
		\item[] $ctr_{x0} := 0$ // Persistent in-memory counter assigned for level $x < \log{N}$  
		\item[] $ctr_{x1} := 0$ // Persistent in-memory counter assigned for level $x < \log{N}$ 
		\item[] $g := 0 $ // Global Access Counter (number of times write queue has been flushed to the disk)
		\EndProcedure
		\Procedure{Merge\_Levels}{$\phi$}
		\For{x = 1 to $\log{N} - 1$}
		\If{$x \neq \log{N} - 1$} 
		\State $ctr_{next} := (g \bmod 2^{x+1}) \times \beta$
		\Else
		\State $ctr_{next} := (g \bmod 2^{x}) \times \beta$
		\EndIf
		\While{ $q_{x0}.notFull$}
		\If{$ctr_{0} \leq 2^{i}\beta$}
		\State Enqueue($q_{x0}$, readFromMergeBuffer($i, ctr_{x0}$)) 
		\State $ctr_{x0} = (ctr_{x0} +1) \bmod 2^{x} $
		\Else
		\State Enqueue($q_{x0}$, fake)
		\EndIf
		\EndWhile
		
		\While{ $q_{x1}.notFull$}
		\If{$ctr_{x1} \leq 2^{i}\beta$}
		\State Enqueue($q_{x1}$, readFromMergeBuffer($i, ctr_{x1} + 2^{x} \times \beta$)) 
		\State $ctr_{x1} = (ctr_{x1} +1) \bmod 2^{x}$
		
		\Else
		\State Enqueue($q_{x1}$, fake)
		\EndIf
		\EndWhile
		
		
		\For{y = 1 to $\beta$}
		\State $b_0 = q_{x0}.peek$
		\State $b_1 = q_{x1}.peek$
		\If{$i \neq \log{N} - 1$}
		\If {$b_0.add < b_1.add$}
		\State $b$ = Dequeue($q_{x0}$)
		\ElsIf {$b_0.add = b_1.add$}
		\State  $b$ = Dequeue($q_{x0}$)
		\State (discard $b_1$ from $q_{x1}$)
		\Else
		\State $b$ = Dequeue($q_{x1}$)
		\EndIf
		\State writeNextToWriteBuffer($x+1, ctr_{next}, b$)
		\Else
		\If{$b_0.add, b_1.add \neq ctr_{next}$}
		\State Reencrypt($i, ctr_{next}$)
		\Else
		\If {$b_0.add < b_1.add$}
		\State $b$ = Dequeue($q_{0}$)
		\ElsIf {$b_0.add = b_1.add$}
		\State  $b$ = Dequeue($q_{0}$)
		\State (discard $b_1$ from $q_{1}$)
		\Else
		\State $b$ = Dequeue($q_{1}$)
		\EndIf
		\State writeToLastLevelBuffer($x+1, ctr_{next}, b$)
		
		\EndIf
		\EndIf						
		\State $ctr_{next} = ctr_{next} + 1$	
		\EndFor
		\EndFor
		\EndProcedure
		%\end{scriptsize}							
	\end{algorithmic}
\end{algorithm}
%

\begin{algorithm}[th!]
	\caption{$\mathsf{Determine\_Level(g,c)}$}\label{det_level}
	%\begin{scriptsize}
	\begin{algorithmic}[1]
		\footnotesize
		%	\begin{footnotesize}
		\State $flush_i = 0$ // Number of subsequent write queue flushes $x$ spent in level $i$ after being flushed to the top level	
		\State $flush_{sum} = 0$  	
		\State $i = 0$
		\While{$flush_{sum} \leq g - c$}
		\If{$\floor{c/2^{i}}\bmod 2 = 0$}
		\State	($x$ was written to generation 0 in level $i$)
		\State $flush_i = 3 \times 2^{i}$
		\Else
		\State ($x$ was written to generation 1 in level $i$)
		\State $flush_i = 2 \times 2^{i}$
		\EndIf			 	
		\State $i = i+1$ 	
		\State $flush_{sum} = flush_{sum} + flush_i$ 
		\EndWhile
		\State Return $i-1$
	\end{algorithmic}
	%\end{scriptsize}
\end{algorithm}


\begin{algorithm}[th!]
	\caption{$\mathsf{SqORAM\_Access}$}\label{rw_algo}
	\begin{algorithmic}[1]
		\footnotesize
		\Function{$\mathsf{SqORAM\_read}$}{$b$}
		\State $root \gets $ Get root node of ATM from memory
		\State $ATM.path \gets $ Get root to leaf path containing entry for $b$
		\While{not at leaf}
		\State $child\_num = ATM.path.nextNode.id$
		\State $l\_ctr \gets \mathsf{root.getVal(child\_num)}$
		\State $child\_level \gets \mathsf{Determine\_Level(g, l\_ctr)}$
		\State $child \gets$ Get Child node from $child\_level$	
		\State $root = child$
		\EndWhile
		
		\State $l\_ctr \gets \mathsf{root.getVal(b)}$
		\State $level \gets \mathsf{Determine\_Level(g, l\_ctr)}$			
		\State $loc\_in\_level \gets \mathsf{level.bufferMap.query}$
		\State $blk \gets$ Read block from $loc\_in\_level$			
		\State \Return $blk$
		\EndFunction
		\Function{$SeqORAM\_write$}{$b,d$}
		\State $\mathsf{WriteQueue.push(b,d)}$
		\State $ATM.path\gets$ Root to leaf path containing entry for $b$
		\State $ATM.node = ATM.path.leafNode$
		\State $\mathsf{ATM.node.update(b,g+1)}$
		\While {not at root}
		\State $\mathsf{WriteQueue.push(ATM.node.id, 
			ATM.node.data)}$
		\State $ATM.node = ATM.path.node.parent$
		\EndWhile
		\item[] // Flush contents of Write Queue sequentially to top level write buffer
		\If {$WriteQueue.full$}
		
		\State $\mathsf{merge\_deamortized()}$
		\EndIf
		\EndFunction
	\end{algorithmic}
\end{algorithm}
%\smallskip




\begin{theorem}[Invariant 1]
	%\label{thm:correctness}
	Algorithm~\ref{merge_level} ensures that all real data blocks from the merge and write buffers of level $i-1$ (for any $i \leq logN$) will be merged in ascending order of their logical addresses and written to level $i$, within $2^{i}\beta$ accesses.
	
	
\end{theorem}

\BPF
%

W.l.o.g. consider that at a particular stage of the merge, $x \leq 2^{i-1}\beta$ blocks have been written from the {\em write buffer} of level $i-i$ and $y \leq 2^{i-1}\beta$ blocks have been written from the {\em merge buffer} of level $i-1$ to level $i$. Since, none of the buffers have been read entirely ($ctr_{w}, ctr_{m} \leq 2^{i-1}\beta$), both $q_w$ and $q_m$ will contain only real blocks at this stage. Now, consider that in subsequent $2^{i-1}\beta - y$ accesses, all remaining blocks from the level $i-1$ merge buffer are written to level $i$ --  a similar argument holds if blocks from the write buffer are written to level $i$ instead. In this case, $q_m$ will contain fake blocks for the remaining $2^{i-1}\beta - x$ accesses (Step 13).  

Since fake blocks invariably have logical address $N+1$ (greater than the logical address of any real data block), the next $2^{i-1}\beta - x$ 
writes will be from $q_w$ (Step 23), until both $q_w$ and $q_m$ contain fake blocks. Further, either of the buffers in level $i-1$ can contain at most $2^{i-1}\beta$ real blocks and 
fake blocks can be added to $q_w$ only after all real data blocks 
have been written (Step 7). Thus, the remaining real blocks from the write buffer will be necessarily written to level $i$ within the next $2^{i-1}\beta - x$ accesses.
\EPF

\begin{theorem}[Security]
	Algorithm~\ref{merge_level} ensures that during the merge all writes to level $i$ are 
	uncorrelated and indistinguishable, independent of the logical block addresses.
\end{theorem}

\BPF 
It is straightforward to see that while merging the buffers of levels $i-1$ and writing to level $i$ (for any $i \leq logN $), the only step observable to the adversary is Step 24 (Algorithm~\ref{merge_level}). The rest of the steps involve reads or in-memory operations that are not visible to the adversary. 

Step 24 performs a write to the {\em next} block in sequence to the write buffer in level $i$, irrespective of the logical block address and content. Also,  invariably the the process is continued until $2^{i}\beta$ blocks have been written (Step 1). In case, the number 
of real data blocks is less than $2^{i}\beta$, {\em fake} blocks are written instead. Semantic security ensures that fake blocks are indistinguishable from real data blocks.

\EPF


\begin{theorem}[Write access complexity]
	The amortized write access complexity of {\sys} is $\O{\log{N}}$ where $N$ is the number of blocks in the ORAM.
\end{theorem}

\BPF
First, note that during construction of level $i$, $2^{i-1}$ buckets each in the write buffer and the merge buffer in level $i-1$ are merged and written to level $i$. For the merge $2^{i}$ buckets in total have to be read from level 
$i-1$ {\em exactly once} while $2^{i}$ buckets are 
written {\em exactly once} to level $i$. Further, 
constructing the B-tree map for the write buffer in level $i$  requires writing $2 \times 2^{i}$ blocks. Level construction for level $i$ can thus be performed with $\O{2^{i}}$ 
accesses. 

Since each level is exponentially larger than the previous level, level $i$ is constructed only after $2^{i} \times \beta$ writes. The amortized write access complexity can then be derived as:

%\begin{center}
%		$\sum\limits_{i=0}^{log_{2}{N/B}} \frac{\O{2^{i}}}{2^{i} \times \beta} =\O{\log{N}}$
%\end{center}

\EPF


\begin{theorem}[Seek analysis]
	The number of disk seeks performed by {\sys} for level reshuffles across $\log{N}$ levels, where $N$ is the number of blocks in the ORAM, amortized over the number of writes is $\frac{4\log{N}}{ \beta}$.
\end{theorem}

\begin{proof}
	Consider the process of merging level $i-1$ buffers and writing to level $i$ as per Algorithm \ref{merge_level}. 
	For the merge at least $M > 2 \times \beta$ blocks of memory is required -- to store two buckets entirely, and compare them in linear time. 
	
	First, blocks are read {\em sequentially} from the merge buffer and the write buffer of level $i-1$ into the in-memory queues, $q_m$ and $q_w$  respectively, until the queues are full. Observe that filling up the queues requires only two disk seeks overall -- to place the head at the starting location of the write buffer and then the merge buffer. After the queues are full, $\beta$ blocks are written to the write buffer of level $i$ {\em sequentially}, which requires {\em one} disk seek. Finally, a leaf node is added to the corresponding buffer B-tree map with entries for block that are written to the bucket, and the parent node(s) of the leaf node are updated in memory. If required, the parent node(s) are flushed to the disk and written {\em sequentially} after the leaf node. This requires 1 seek in total.
	
	
	Overall, writing a bucket containing $\beta$ blocks to the write buffer requires 4 seeks in total. Since, the write buffer of level $i$ contains $2^{i}$ buckets, the total number of seeks to complete filling up the write buffer is $4 \times 2^{i}$. Also, the write buffer in level $i$  gets filled up after $2^{i}$ writes. Thus, the number seeks for all level reconstructions amortized over the number of writes is:
	
	\begin{center}
		$s = \sum\limits_{i=0}^{log_{k}{N/B}} \frac{4 \times 2^{i}}{2^{i} \beta} = \frac{4 \log{N}}{\beta} $
	\end{center}
	
\end{proof}

%

\begin{algorithm}[th!]
	\caption{$\mathsf{Determine\_Level(g,c)}$}\label{det_level}
	%\begin{scriptsize}
	\begin{algorithmic}[1]
		\footnotesize
		%	\begin{footnotesize}
		\State $flush_i = 0$ // Number of subsequent write queue flushes $x$ spent in level $i$ after being flushed to the top level	
		\State $flush_{sum} = 0$  	
		\State $i = 0$
		\While{$flush_{sum} \leq g - c$}
		\If{$\floor{c/2^{i}}\bmod 2 = 0$}
		\State	($x$ was written to generation 0 in level $i$)
		\State $flush_i = 3 \times 2^{i}$
		\Else
		\State ($x$ was written to generation 1 in level $i$)
		\State $flush_i = 2 \times 2^{i}$
		\EndIf			 	
		\State $i = i+1$ 	
		\State $flush_{sum} = flush_{sum} + flush_i$ 
		\EndWhile
		\State Return $i-1$
	\end{algorithmic}
	%\end{scriptsize}
\end{algorithm}


\begin{algorithm}[th!]
	\caption{$\mathsf{SqORAM\_Access}$}\label{rw_algo}
	\begin{algorithmic}[1]
		\footnotesize
		\Function{$\mathsf{SqORAM\_read}$}{$b$}
		\State $root \gets $ Get root node of ATM from memory
		\State $ATM.path \gets $ Get root to leaf path containing entry for $b$
		\While{not at leaf}
		\State $child\_num = ATM.path.nextNode.id$
		\State $l\_ctr \gets \mathsf{root.getVal(child\_num)}$
		\State $child\_level \gets \mathsf{Determine\_Level(g, l\_ctr)}$
		\State $child \gets$ Get Child node from $child\_level$	
		\State $root = child$
		\EndWhile
		
		\State $l\_ctr \gets \mathsf{root.getVal(b)}$
		\State $level \gets \mathsf{Determine\_Level(g, l\_ctr)}$			
		\State $loc\_in\_level \gets \mathsf{level.bufferMap.query}$
		\State $blk \gets$ Read block from $loc\_in\_level$			
		\State \Return $blk$
		\EndFunction
		\Function{$SeqORAM\_write$}{$b,d$}
		\State $\mathsf{WriteQueue.push(b,d)}$
		\State $ATM.path\gets$ Root to leaf path containing entry for $b$
		\State $ATM.node = ATM.path.leafNode$
		\State $\mathsf{ATM.node.update(b,g+1)}$
		\While {not at root}
		\State $\mathsf{WriteQueue.push(ATM.node.id, 
			ATM.node.data)}$
		\State $ATM.node = ATM.path.node.parent$
		\EndWhile
		\item[] // Flush contents of Write Queue sequentially to top level write buffer
		\If {$WriteQueue.full$}
		
		\State $\mathsf{merge\_deamortized()}$
		\EndIf
		\EndFunction
	\end{algorithmic}
\end{algorithm}
%\smallskip




%\begin{customthm}{1}
% The amortized {\sys} construction provides write access pattern indistinguishability.
%\end{customthm}
%
%\begin{proofsketch}
%%
%The proof follows straighforwardly by construction.  Given two equal length
%access patterns, $A = {w_1, w_2, \ldots w_i}$ and $B = {x_1, x_2, \ldots
%x_i}$, $i$ encrypted writes are first added to the write queue irrespective
%the logical addresses.  When the write queue is flushed, it triggers level
%reconstructions independent of the contents of the write queue.
% 
%During the level reconstructions, blocks from two buckets are merged
%together on the basis of their logical addresses.  Since reads are not
%observable, the buckets that are being merged are not known to the
%adversary.  The order in which the merged buckets are written is independent
%of the result of the merge.  More specifically, during a merge for level
%$i$, an adversary observes buckets always written in the order of 1 to
%$2^{i}$ irrespective of the contents of the buckets.  Since, blocks are
%written reencrypted during a merge, the semantic security of the encryption
%scheme provides indistinguishability between the blocks written to a bucket
%after the merge.  Thus, observing write traces for $i$ subsequent writes, an
%adversary can only do negligibly better than purely guessing whether $A$ or
%$B$ was executed.
%% 
%\end{proofsketch}
%

\begin{theorem}[De-amortized Security]
	Algorithm~\ref{merge_level_deamortized} ensures that during the merge all writes to level $i$ are 
	uncorrelated and indistinguishable, independent of the logical block addresses.
\end{theorem}

\BPF
It is straightforward to see that while executing Algorithm \ref{merge_level_deamortized}, the only steps visible to the adversary are Step 29, 32 and 41. 

Step 29 and 41 combined perform a write to the {\em next} block in sequence to the write buffer in every level of the ORAM, irrespective of the logical block address and content. Also,  invariably the the process is continued until $\beta$ blocks have been written {\em sequentially} to the write buffer of every level (Step 18). In case, there are less than $\beta$ real data blocks that can be written {\em fake} blocks are written instead. Semantic security ensures that fake blocks are indistinguishable from real data blocks.

Step 32 re-encrypts the content of the {\em next} block in sequence in the last level buffer. Due to semantic security, re-encryption is indistinguishable from a real write, thus rending this step indistinguishable from Step 41.  


\EPF


\begin{theorem}[De-amortized Correctness]
	Algorithm~\ref{merge_level_deamortized} ensures that by the time the write buffer of level $i < \log{N}$ is full, all real data blocks from the merge buffer of level $i$ have been written to level $i+1$.
\end{theorem}

\begin{proof}
	Every successive execution of Algorithm \ref{merge_level_deamortized} writes $\beta$ to the write buffer of level $i$ {\em sequentially}. At the same time, $\beta$ blocks are written from the merge buffer of level $i$ to the write buffer in level $i+1$. Note that within exactly $2^{i+1}$ successive executions of Algorithm \ref{merge_level_deamortized}, the write buffer of level $i$ will be full. But within the same time, $2^{i+1}\beta$ blocks will have been written from the merge buffer of level to level $i+1$ (Line 18 - 29).
	From Theorem \ref{thm:correctness}, all real blocks from the merge buffer of level $i$ will necessarily be written to level $i+1$ within these $2^{i+1}\beta$ writes. This ensures that when the buffer are switched, all valid content from the merge buffer of level $i$ will have been written to level $i+1$ thus preventing data loss due to overwriting.  
\end{proof}

\begin{algorithm}[]
	\caption{$\mathsf{merge\_deamortized}$}\label{merge_level_deamortized}
	\begin{algorithmic}[1]
		%\begin{scriptsize}
		\footnotesize
		\Procedure{Init}{$\phi$}
		\item[] $q_{x0} := \phi$ // Persistent in-memory queue of size $\beta$ assigned for level $x < \log{N}$
		\item[] $q_{x1} := \phi$ // Persistent in-memory queue of size $\beta$ assigned for level $x < \log{N}$
		\item[] $ctr_{x0} := 0$ // Persistent in-memory counter assigned for level $x < \log{N}$  
		\item[] $ctr_{x1} := 0$ // Persistent in-memory counter assigned for level $x < \log{N}$ 
		\item[] $g := 0 $ // Global Access Counter (number of times write queue has been flushed to the disk)
		\EndProcedure
		\Procedure{Merge\_Levels}{$\phi$}
		\For{x = 1 to $\log{N} - 1$}
		\If{$x \neq \log{N} - 1$} 
		\State $ctr_{next} := (g \bmod 2^{x+1}) \times \beta$
		\Else
		\State $ctr_{next} := (g \bmod 2^{x}) \times \beta$
		\EndIf
		\While{ $q_{x0}.notFull$}
		\If{$ctr_{0} \leq 2^{i}\beta$}
		\State Enqueue($q_{x0}$, readFromMergeBuffer($i, ctr_{x0}$)) 
		\State $ctr_{x0} = (ctr_{x0} +1) \bmod 2^{x} $
		\Else
		\State Enqueue($q_{x0}$, fake)
		\EndIf
		\EndWhile
		
		\While{ $q_{x1}.notFull$}
		\If{$ctr_{x1} \leq 2^{i}\beta$}
		\State Enqueue($q_{x1}$, readFromMergeBuffer($i, ctr_{x1} + 2^{x} \times \beta$)) 
		\State $ctr_{x1} = (ctr_{x1} +1) \bmod 2^{x}$
		
		\Else
		\State Enqueue($q_{x1}$, fake)
		\EndIf
		\EndWhile
		
		
		\For{y = 1 to $\beta$}
		\State $b_0 = q_{x0}.peek$
		\State $b_1 = q_{x1}.peek$
		\If{$i \neq \log{N} - 1$}
		\If {$b_0.add < b_1.add$}
		\State $b$ = Dequeue($q_{x0}$)
		\ElsIf {$b_0.add = b_1.add$}
		\State  $b$ = Dequeue($q_{x0}$)
		\State (discard $b_1$ from $q_{x1}$)
		\Else
		\State $b$ = Dequeue($q_{x1}$)
		\EndIf
		\State writeNextToWriteBuffer($x+1, ctr_{next}, b$)
		\Else
		\If{$b_0.add, b_1.add \neq ctr_{next}$}
		\State Reencrypt($i, ctr_{next}$)
		\Else
		\If {$b_0.add < b_1.add$}
		\State $b$ = Dequeue($q_{0}$)
		\ElsIf {$b_0.add = b_1.add$}
		\State  $b$ = Dequeue($q_{0}$)
		\State (discard $b_1$ from $q_{1}$)
		\Else
		\State $b$ = Dequeue($q_{1}$)
		\EndIf
		\State writeToLastLevelBuffer($x+1, ctr_{next}, b$)
		
		\EndIf
		\EndIf						
		\State $ctr_{next} = ctr_{next} + 1$	
		\EndFor
		\EndFor
		\EndProcedure
		%\end{scriptsize}							
	\end{algorithmic}
\end{algorithm}

%\begin{customthm}{2}
% The deamortized {\sys} construction provides write access pattern indistinguishability.
%\end{customthm}
%
%\begin{proofsketch}
%%
%The deamortized construction makes two changes to the amortized
%construction: an extra buffer is added to each level and the ATM is stored
%within the ORAM.  First, the merging in this case proceeds deterministically
%and independent of the blocks being merged -- buckets in generation 0 of the
%write buffer of a level are written sequentially before the buckets in
%generation 1.  Once the write buffer is full, it is switched to the merge
%buffer.  Note that buckets are only {\em read} from the merge buffer and
%merged in memory.  Since reads are not observable and buckets written after
%the merge are encrypted with semantic security, the outcome of the merge is
%not determinable by an adversary.
%  
%Further, since reads are not observable, using the ATM during reads to
%reduce the number of levels searched for a block does not provide any
%additional information to the adversary.  Finally, the ATM blocks are
%written to the write queue indistinguishably from data blocks due to
%semantic security of the encryption.
%%
%\end{proofsketch}
%
%


==> model.tex <==
\section{Model}
\label{seqoram:model}
%
% \begin{figure}
% \centering
% \includegraphics[scale=0.18]{figures/seqoram_model.eps}
% \caption{{\sys} deployment model. {\sys} maps data from a logical volume 
% to a storage device. The write to the storage device is monitored by a {\em multi-snapshot} 
% adversary that can access the device after every write operation.\label{seqoram_model}}
% \end{figure}


\smallskip
\noindent
{\bf Deployment.~} Data originating from a logical volume (which 
may support a filesystem on top) is written encrypted to a storage device
(either local disk or network storage). 

\smallskip
\noindent
{\bf Adversary.~} The main write-only ORAM adversary is a {\em multi-snapshot} adversary
that can access the storage device after one or more write operations. 

The adversary may save device snapshots -- including device specific
information, filesystem metadata and bits stored in each block -- and
compare these snapshots with the current state in an attempt to learn about
the location of the written information.  The adversary does not however
monitor device reads or accesses to client DRAM in between writes to the
main device.

\smallskip
\noindent
{\bf Write access patterns.~}
%
{\em Access patterns} are informally defined as an {\em ordered sequence} of
logical block writes.

\smallskip
\noindent
{\bf Write traces.~}
%
{\em Write trace} are informally defined as the actual modifications to physical blocks
due to the execution of a corresponding {\em access pattern}.


\smallskip
\noindent
{\bf Security.~} 
%
{\sys} uses the security model from \cite{hive}.
Informally, a write-only ORAM is secure if it provides {\em write access pattern indistinguishability} against a computationally bounded adversary. 

%Write access pattern indistinguishability has been formally~\cite{hive} defined as: 
%For a device with $N$ physical blocks, given two access patterns of equal
%length $\mathcal{O}_0 = \{a_{1}, a_{2}, \ldots , a_{i}\}$ and $\mathcal{O}_1
%= \{b_{1}, b_{2}, \ldots , b_{i}\}$ and a random {\em write trace},
%$\mathcal{W} = \{w_{1}, w_{2}, \ldots , w_{i}\}$ with $w_i \in N$,
%$\mathcal{O}_0$ is said to be indistinguishable from $\mathcal{O}_1$ iff. 
%there exists a function $\epsilon$, negligible in the security parameter $s$ such that

%\begin{center}
%    $Pr[\mathcal{W}| \mathcal{O}_{0}] - Pr[\mathcal{W}| \mathcal{O}_{1}] < \epsilon(s)$
%\end{center}
%
%Here $Pr[\mathcal{W} | \mathcal{O}_{i}], i =0,1$ is the probability that 
%$\mathcal{W}$ is the sequence of writes caused to the disk by executing $\mathcal{O}_{i}$.
% 


% \todo{where did you get this definition from? doesn't epsilon need to be
% negligible?}
% 
% \todo{can you make this a proper \\definition}

% \smallskip
% \noindent
% {\bf Security.~} 
% %
% . \todo{can we then remove the
% definition above?}


\smallskip
\noindent
{\bf Minimizing I/O latency.~}
%
A main goal of {\sys} is to reduce the latency of access for each ORAM operation
and specifically the number of disk seeks per access.

% . Latency of accesses to mechanical storage disks are 
% composed of three components: seek time, rotational latency and data transfer time.
% Out of these, the seek time is the most expensive component and orders of magnitude 
% slower than the data transfer rate. 

% To ensure obliviousness, individual ORAM accesses may 
% need to perform multiple disk I/Os (as established by the 
% lower bound from \cite{goldreich}). Thus, reducing the number of 
% seeks for performing these additional disk I/Os is essential to optimize the latency of each access. 

% \todo{very confusing --
% what is "seek time between accesses"?, also doesn't this replicate the text
% below}

% \smallskip
% \noindent
% {\bf Evaluation metric.~ }
%
Note that this is orthogonal to the typical ORAM performance metrics which
involve just optimizing the bandwidth per access.  
% of access -- the additional I/O that needs to be performed per operation for 
% obliviousness. 
Optimizing bandwidth is important when ORAMs 
are deployed in networks but seeks tend to dominate for local storage.
%  storage since transferring data over high latency networks 
% are expensive. However, data transfer rates on local 
% storage disks are much faster than over networks. Further, 
% as discussed above, seek times for storage disks dominate data transfer rates by 
% orders of magnitude. 
% Thus, additional I/O does not drastically affect performance 
% {\em if} seeks in between the additional accesses are minimized. Consequently, 
% Thus, in addition to access complexity, 
% {\sys} aims to reduce the number of required device seeks per access, 

\smallskip
\noindent
{\bf Logical vs. physical complexity.~}
% 
Existing ORAMs define access complexity as the number of logical blocks of
data accessed per I/O.  This allows optimzations by using logical blocks of
smaller size~\cite{Shi_obliviousram,pathoram}.  However, it is important to
note that standard off-the-shelf storage block-based storage device can
access data only in units of physical blocks (sectors).  For example,
accessing a 256 byte logical block still entails accessing the corresponding
4KB disk block from the disk.  Thus, in the context of locally-deployed
block-based devices, it is important to also measure the complexity of the
physical block accesses per ORAM I/O.

%\smallskip
%\noindent
%{\bf State-of-the-art.~}
%%
%The most bandwidth-efficient write-only ORAM to date is
%HIVE-ORAM~\cite{hive}.  It has a physical block read complexity (number of
%physical blocks read) of $\order{log_{\beta}N}$ and a physical write
%complexity (number of blocks written) of $\order{log_{\beta}^{2}N}$ where
%$\beta= B/|addr|$, $B$ is the physical block size in bytes and $|addr|$ is
%the size of one physical block address in bytes.


